Consistency-preserving Visual Question Answering in Medical Imaging

Visual Question Answering (VQA) models take an image and a natural-language question as input and infer the answer to the question. Recently, VQA systems in medical imaging have gained popularity thanks to potential advantages such as patient engagement and second opinions for clinicians. While most research efforts have been focused on improving architectures and overcoming data-related limitations, answer consistency has been overlooked even though it plays a critical role in establishing trustworthy models. In this work, we propose a novel loss function and corresponding training procedure that allows the inclusion of relations between questions into the training process. Specifically, we consider the case where implications between perception and reasoning questions are known a-priori. To show the benefits of our approach, we evaluate it on the clinically relevant task of Diabetic Macular Edema (DME) staging from fundus imaging. Our experiments show that our method outperforms state-of-the-art baselines, not only by improving model consistency, but also in terms of overall model accuracy. Our code and data are available at https://github.com/sergiotasconmorales/consistency_vqa.

==> sections/material.tex <==
\begin{figure}[]
\begin{center}
\includegraphics[width=\textwidth]{images/boxplots.pdf}
\caption{Effect of the variation of the hyperparameters $\lambda$ and $\gamma$, for each metric. The first 5 rows refer to accuracy for all questions (overall), for main questions (main) and for sub-questions (whole, macula and regions). The last two rows correspond to the consistency. In general, a higher value of $\lambda$ leads to a higher consistency, which is the expected behavior. High values of both parameters can produce a decrease in the accuracy of main questions.}
\label{fig:method}
\end{center}
\end{figure}

\begin{figure}[]
\begin{center}
\includegraphics[width=\textwidth]{images/examples_supplementary_ext.pdf}
\caption{Additional qualitative examples from the DME dataset. Inconsistent answers are highlighted in red. A more consistent behavior is observed in our method in comparison to the baselines (rows 1-2). Even though our method can make mistakes (rows 3-4), it also shows an improvement in the performance on main questions (rows 5-6).}
\label{fig:method}
\end{center}
\end{figure}
